A Cognitive Study on Semantic Similarity Analysis of Large Corpora: A Transformer-based Approach

Semantic similarity analysis and modeling is a fundamentally acclaimed task in many pioneering applications of natural language processing today. Owing to the sensation of sequential pattern recognition, many neural networks like RNNs and LSTMs have achieved satisfactory results in semantic similarity modeling. However, these solutions are considered inefficient due to their inability to process information in a non-sequential manner, thus leading to the improper extraction of context. Transformers function as the state-of-the-art architecture due to their advantages like non-sequential data processing and self-attention. In this paper, we perform semantic similarity analysis and modeling on the U.S Patent Phrase to Phrase Matching Dataset using both traditional and transformer-based techniques. We experiment upon four different variants of the Decoding Enhanced BERT - DeBERTa and enhance its performance by performing K-Fold Cross-Validation. The experimental results demonstrate our methodology's enhanced performance compared to traditional techniques, with an average Pearson correlation score of 0.79.

==> name.tex <==
One of the significant solutions proposed to tackle the task of semantic similarity is Siamese Neural Networks, also abbreviated as SNNs \cite{koch2015siamese}. In a broader perspective, siamese neural networks are those neural networks that consist of two or more analogous sub-networks. The sub-networks have similar parameters and weights and are mirrored in parameter updating. Due to their structural composition and robustness to class imbalance, Siamese Neural Networks are used to estimate the similarity between two data points. Keeping these points in view, some of the solutions involving the usage of SNNs are described below:
